X2CT-CLIP: Enable Multi-Abnormality Detection in Computed Tomography from Chest Radiography via Tri-Modal Contrastive Learning

Computed tomography (CT) is a key imaging modality for diagnosis, yet its clinical utility is marred by high radiation exposure and long turnaround times, restricting its use for larger-scale screening. Although chest radiography (CXR) is more accessible and safer, existing CXR foundation models focus primarily on detecting diseases that are readily visible on the CXR. Recently, works have explored training disease classification models on simulated CXRs, but they remain limited to recognizing a single disease type from CT. CT foundation models have also emerged with significantly improved detection of pathologies in CT. However, the generalized application of CT-derived labels on CXR has remained illusive. In this study, we propose X2CT-CLIP, a tri-modal knowledge transfer learning framework that bridges the modality gap between CT and CXR while reducing the computational burden of model training. Our approach is the first work to enable multi-abnormality classification in CT, using CXR, by transferring knowledge from 3D CT volumes and associated radiology reports to a CXR encoder via a carefully designed tri-modal alignment mechanism in latent space. Extensive evaluations on three multi-label CT datasets demonstrate that our method outperforms state-of-the-art baselines in cross-modal retrieval, few-shot adaptation, and external validation. These results highlight the potential of CXR, enriched with knowledge derived from CT, as a viable efficient alternative for disease detection in resource-limited settings.

==> tables/external_val_tab.tex <==
\begingroup  % Start temporary scope
    \setlength\dashlinedash{0.3pt}     % Make dashes very small (almost dots)
    \setlength\dashlinegap{1.5pt}      % Increase gap to make it look like dots
    \setlength\arrayrulewidth{0.3pt}   % Adjust thickness for a finer look

    \begin{table}[ht!]
        \centering
        \caption{External validation in restricted data regime. $^*$indicates statistical significance based on the DeLong test statistics at $5\%$ significance level compared to the closest baseline.}

            \begin{tabular}{cc:cc:cc:cc:cc}  % Fixed column count
                \thickhline
                \multirow{3}{*}{Method} & \multirow{3}{*}{Backbone} & \multicolumn{4}{c:}{\textbf{RadChest-CT}(External)} & \multicolumn{4}{c}{\textbf{MIMIC-CT}(External)}\\
                & & \multicolumn{2}{c:}{FS@5\%} & \multicolumn{2}{c:}{FS@10\%} & \multicolumn{2}{c:}{FS@5\%} & \multicolumn{2}{c}{FS@10\%}\\
                & & AUC$\uparrow$ & PR$\uparrow$ & AUC$\uparrow$ & PR$\uparrow$ & AUC$\uparrow$ & PR$\uparrow$ & AUC$\uparrow$ & PR$\uparrow$ \\  
                \hline
                \multirow{2}{*}{GLoRIA} & ResNet & 0.694 & 0.432 & 0.692 & 0.431 & 0.709 & 0.313 & 0.726 & 0.339\\
                                          & DenseNet & 0.712 & 0.496 & 0.719 & 0.497 & 0.692 & 0.316 & 0.710 & 0.330\\
                \hdashline[1pt/2pt]
                \multirow{2}{*}{MedCLIP} & ResNet & 0.684 & 0.441 & 0.689 & 0.453 & 0.754 & 0.365 & 0.770 & 0.388\\
                                          & Swin & 0.700 & 0.457 & 0.701 & 0.455 & 0.752 & 0.383 & 0.764 & 0.408\\
                \hdashline[1pt/2pt]
                \multirow{2}{*}{CXRCLIP} & ResNet & 0.721 & 0.512 & 0.721 & 0.505 & 0.684 & 0.314 & 0.688 & 0.304\\
                                          & Swin & 0.722 & 0.513 & 0.719 & 0.512 & 0.639 & 0.242 & 0.665 & 0.272\\  
                \hdashline[1pt/2pt]
                Multi-View & BI-Mamba & 0.663 & 0.412 & 0.666 & 0.424 & 0.742 & 0.360 & 0.733 & 0.369\\
                \hline
                \multirow{2}{*}{Ours} & ResNet & $\textbf{0.735}^*$ & $\textbf{0.559}$ & \underline{0.728} & \underline{0.555} & $\textbf{0.790}^*$ & \textbf{0.434} & \underline{0.766} & \underline{0.412}\\
                                      & Swin & \underline{0.731} & \underline{0.555} & $\textbf{0.733}^*$ & \textbf{0.558} & \underline{0.760} & \underline{0.412} & $\textbf{0.794}^*$ & \textbf{0.438}\\
                \thickhline
            \end{tabular}
        \label{tab:external_val}
    \end{table}
\endgroup  % End temporary scope, restore default tabcolsep
% RADCHEST_CT_PURE_INTERNAL

==> tables/task_adaptation_tab.tex <==
\begingroup  % Start temporary scope
    \setlength\dashlinedash{0.3pt}     % Make dashes very small (almost dots)
    \setlength\dashlinegap{1.5pt}      % Increase gap to make it look like dots
    \setlength\arrayrulewidth{0.3pt}   % Adjust thickness for a finer look

    \begin{table}[ht!]
        \centering
        \caption{Few-shot adaptation. $^*$indicates statistical significance based on the DeLong test statistics at $5\%$ significance level compared to the closest baseline.}
            \begin{tabular}{cc:cc:cc:cc:cc}  % Fixed column count
                % \specialrule{0.05em}{0em}{0em}  % Custom top rule
                \thickhline
                \multirow{3}{*}{Method} & \multirow{3}{*}{Backbone} & \multicolumn{4}{c:}{\textbf{RadChest-CT}} & \multicolumn{4}{c}{\textbf{CT-RATE}} \\
                & & \multicolumn{2}{c:}{FS@20\%} & \multicolumn{2}{c:}{FS@50\%} & \multicolumn{2}{c:}{FS@20\%} & \multicolumn{2}{c}{FS@50\%} \\
                & & AUC$\uparrow$ & PR$\uparrow$ & AUC$\uparrow$ & PR$\uparrow$ & AUC$\uparrow$ & PR$\uparrow$ & AUC$\uparrow$ & PR$\uparrow$ \\  
                \hline
                \multirow{2}{*}{GLoRIA} & ResNet & 0.870 & 0.629 & 0.869 & 0.619 & 0.784 & 0.455 & 0.785 & 0.457\\
                                          & DenseNet & 0.878 & 0.652 & 0.880 & 0.644 & 0.815 & 0.525 & 0.816 & 0.524\\
                \hdashline[1pt/2pt]
                \multirow{2}{*}{MedCLIP} & ResNet & 0.880 & 0.649 & 0.876 & 0.626 & 0.799 & 0.494 & 0.799 & 0.497\\
                                          & Swin & 0.879 & 0.644 & 0.878 & 0.631 & 0.804 & 0.507 & 0.787 & 0.473\\
                \hdashline[1pt/2pt]
                \multirow{2}{*}{CXRCLIP} & ResNet & 0.878 & 0.670 & 0.881 & 0.669 & 0.826 & 0.549 & 0.828 & 0.551\\
                                          & Swin & 0.879 & 0.671 & 0.883 & 0.669 & 0.828 & 0.549 & 0.831 & 0.553\\  
                \hdashline[1pt/2pt]
                Multi-View & BI-Mamba & 0.871 & 0.641 & 0.869 & 0.633 & 0.772 & 0.43 & 0.779 & 0.448\\
                \hline
                \multirow{2}{*}{Ours} & ResNet & \underline{0.887} & \textbf{0.683} & \underline{0.893} & \underline{0.687} & \underline{0.840} & \underline{0.565} & \underline{0.843} & \underline{0.577}\\
                                      & Swin & $\textbf{0.888}^*$ & \underline{0.681} & $\textbf{0.894}^*$ & \textbf{0.692} & $\textbf{0.841}^*$ & \textbf{0.566} & $\textbf{0.847}^*$ & \textbf{0.579} \\
                \thickhline
            \end{tabular}
        \label{tab:task_adaptation}
    \end{table}
\endgroup  % End temporary scope, restore default tabcolsep


==> tables/xray_ct_retrieval_tab.tex <==
\begingroup  % Start temporary scope
    \setlength{\tabcolsep}{3pt}  % Reduce spacing for this table only
    \setlength\dashlinedash{0.3pt}     % Make dashes very small (almost dots)
    \setlength\dashlinegap{1.5pt}      % Increase gap to make it look like dots
    \setlength\arrayrulewidth{0.3pt}   % Adjust thickness for a finer look

    \begin{table}[ht!]
        \centering
        \caption{CT volume retrieval using CXR. $^1$CT volume retrieval queried by CT report}

\begin{tabular}{cc:cc:cc:cc:cc}
                \thickhline
                \multirow{2}{*}{Method} & \multirow{2}{*}{Model} & \multicolumn{4}{c:}{\textbf{CT-RATE}} & \multicolumn{4}{c}{\textbf{RadChest-CT}}\\
                & & $\text{R}_5\uparrow$ & $\text{R}_{10}\uparrow$ & $\text{AP}_5\uparrow$ & $\text{AP}_{10}\uparrow$ &$\text{R}_5\uparrow$ & $\text{R}_{10}\uparrow$ & $\text{AP}_5\uparrow$ & $\text{AP}_{10}\uparrow$\\
                \hline
                \multirow{2}{*}{MedCLIP} & ResNet & 0.001 & 0.001 & 0.134 & 0.131 & 0.001 & 0.001 & 0.261 & 0.268 \\
                                          & Swin & 0.001 & 0.002 & 0.134 & 0.120 & 0.001 & 0.001 & 0.328 & 0.310 \\
                \hdashline[1pt/2pt]
                \multirow{2}{*}{CXRCLIP} & ResNet & 0.000 & 0.001 & 0.169 & 0.170 & 0.001 & 0.001 & 0.354 & 0.349 \\
                                          & Swin & 0.000 & 0.001 & 0.151 & 0.150 & 0.001 & 0.001 & 0.307 & 0.308 \\
                \hdashline[1pt/2pt]
                CTCLIP$^1$ & 3DViT & 0.030 & 0.055 & 0.264 & 0.261 & - & - & - & - \\
                \hline
                \multirow{2}{*}{Ours} & ResNet & \underline{0.118} & \underline{0.162} & \underline{0.271} & \underline{0.260} & \underline{0.043} & \underline{0.062} & \textbf{0.387} & \underline{0.379} \\
                                      & Swin & \textbf{0.129} & \textbf{0.181} & \textbf{0.277} & \textbf{0.266} & \textbf{0.045} & \textbf{0.063} & \underline{0.382} & \textbf{0.378} \\
                \thickhline
            \end{tabular}
        \label{tab:ct_vol_retrieval}
    \end{table}
\endgroup  % End temporary scope, restore default tabcolsep


==> tables/xray_report_retrieval_tab.tex <==
\begingroup  % Start temporary scope
    \setlength{\tabcolsep}{3pt}  % Reduce spacing for this table only
    \setlength\dashlinedash{0.3pt}     % Make dashes very small (almost dots)
    \setlength\dashlinegap{1.5pt}      % Increase gap to make it look like dots
    \setlength\arrayrulewidth{0.3pt}   % Adjust thickness for a finer look

    \begin{table}[ht!]
        \centering
        \caption{CT report retrieval using CXR. $^1$CT report retrieval queried by CT volume.}
            \begin{tabular}{cc:cc:cc:cc:cc}
                \thickhline
                \multirow{2}{*}{Method} & \multirow{2}{*}{Model} & \multicolumn{4}{c:}{\textbf{CT-RATE}} & \multicolumn{4}{c}{\textbf{MIMIC-CT}}\\
                & & $\text{R}_5\uparrow$ & $\text{R}_{10}\uparrow$ & $\text{AP}_5\uparrow$ & $\text{AP}_{10}\uparrow$ &$\text{R}_5\uparrow$ & $\text{R}_{10}\uparrow$ & $\text{AP}_5\uparrow$ & $\text{AP}_{10}\uparrow$\\
                \hline
                \multirow{2}{*}{MedCLIP} & ResNet & 0.001 & 0.001 & 0.053 & 0.066 & 0.012  & 0.023 & 0.264 & 0.270 \\
                                          & Swin & 0.001 & 0.002 & 0.163 & 0.160 & 0.012  & 0.023 & 0.276 & 0.279 \\
                \hdashline[1pt/2pt]
                \multirow{2}{*}{CXRCLIP} & ResNet & 0.001 & 0.002 & 0.164 & 0.164 & 0.004  & 0.004 & 0.213 & 0.220 \\
                                          & Swin & 0.000 & 0.001 & 0.158 & 0.156 & 0.019  & 0.019 & 0.248 & 0.253 \\
                \hdashline[1pt/2pt]
                CTCLIP$^2$ & 3DViT & 0.029 & 0.051  & 0.241 & 0.239  & - & - & - & - \\
                \hline
                \multirow{2}{*}{Ours} & ResNet & \textbf{0.048} & \underline{0.077} & \textbf{0.280} & \textbf{0.275} & \textbf{0.113}  & \underline{0.141} & \textbf{0.316} & \underline{0.298} \\
                                      & Swin & \underline{0.047} & \textbf{0.078} & \underline{0.278} & \textbf{0.275} & \textbf{0.113}  & \textbf{0.160} & \underline{0.297} & \textbf{0.314} \\
                \thickhline
            \end{tabular}
        \label{tab:ct_report_retrieval}
    \end{table}
\endgroup  % End temporary scope, restore default tabcolsep


